Temporal Analysis of Entity Relatedness and its Evolution using Wikipedia and DBpedia

Many researchers have made use of the Wikipedia network for relatedness and similarity tasks. However, most approaches use only the most recent information and not historical changes in the network. We provide an analysis of entity relatedness using temporal graph-based approaches over different versions of the Wikipedia article link network and DBpedia, which is an open-source knowledge base extracted from Wikipedia. We consider creating the Wikipedia article link network as both a union and intersection of edges over multiple time points and present a novel variation of the Jaccard index to weight edges based on their transience. We evaluate our results against the KORE dataset, which was created in 2010, and show that using the 2010 Wikipedia article link network produces the strongest result, suggesting that semantic similarity is time sensitive. We then show that integrating multiple time frames in our methods can give a better overall similarity demonstrating that temporal evolution can have an important effect on entity relatedness.

==> problems-old.tex <==
\subsection{Problem Statement and Research Contributions}
%We analyse the Evolution of Entity Relatedness using Wikipedia Network to demonstrate how temporal information effect in network analysis. 
In order to demonstrate entity relatedness and its evolution, we divide the problems in to two main problems as the following:

\begin{itemize}
\item Problem 1: How to represent Wikipedia network for the entity relatedness problem? 
\\ 
Wikipedia articles have the links to other Wikipedia articles. Can we use this information to create Wikipedia article link network for the entity relatedness problem. What are the other information provided by Wikipedia that might be benefit to the analysis? How can we correspond a entity to a Wikipedia article? 
How can temporal information be represented in the network?
%What temporal graph representations can be use to reflect the temporal information effects on the entity relatedness.
We propose various temporal models to represent Wikipedia article link network to analyse entity relatedness based on the assumption that closely related entities share the same adjacent nodes in the network. We also analysed if the the in-links and out-links have the same effects to their relatedness.
%\item Question 2.2: Can we apply changes in Wikipedia network to identify relatedness and similarity of entities over time? %How can we understand change in Wikipedia network? 
\\ 
%Based on the proposed Wikipedia network representation, can we use this information to demonstrate the evolution of entity relatedness? First of all, we have to answer the question how we can understand changes in the Wikipedia network and understand the properties of change that can be apply to the entity relatedness problem.
\item Problem 2: What is the method used to find relatedness and its evolution using Wikipedia network?
\\ 
What techniques we can use to find relatedness score of the entities? There might be some articles that link to a lot of the articles that might not be semantically related. For example, the main page, which is the landing page for featured articles and news, is not semantically related to the articles it links to. On the other hand, articles that do not have many links to other pages might have more semantically relation to their links. How can we choose weights to penalise those articles that link to many other unrelated articles?
How temporal information affects relatedness of entities?
%Can we apply changes in Wikipedia network to identify relatedness and similarity of entities over time?
How transient links, links that do not persist over different times, and stable links, links that persist over time respectively, affect the relatedness of the entities? How frequent do the relatedness of entities change?

Towards these questions, we provide graph-based methods for entity relatedness and show how temporal information affect relatedness of entities. We show how entity relatedness develops over time as well as how transient links and stable links affect the relatedness of the entities. We also show how frequently the relatedness of entities change.
\end{itemize}
